Meta-Path-based Fake News Detection Leveraging Multi-level Social Context Information

Fake news, false or misleading information presented as news, has a significant impact on many aspects of society, such as in politics or healthcare domains. Due to the deceiving nature of fake news, applying Natural Language Processing (NLP) techniques to the news content alone is insufficient. The multi-level social context information (news publishers and engaged users in social media) and temporal information of user engagement are important information in fake news detection. The proper usage of this information, however, introduces three chronic difficulties: 1) multi-level social context information is hard to be used without information loss, 2) temporal information is hard to be used along with multi-level social context information, 3) news representation with multi-level social context and temporal information is hard to be learned in an end-to-end manner. To overcome all three difficulties, we propose a novel fake news detection framework, Hetero-SCAN. We use Meta-Path to extract meaningful multi-level social context information without loss. Meta-Path, a composite relation connecting two node types, is proposed to capture the semantics in the heterogeneous graph. We then propose Meta-Path instance encoding and aggregation methods to capture the temporal information of user engagement and produce news representation end-to-end. According to our experiment, Hetero-SCAN yields significant performance improvement over state-of-the-art fake news detection methods.

==> section/1_introduction.tex <==
\section{Introduction}

The wide dissemination of fake news has become a major social problem in the world.
The most recent and infamous distribution of fake news was in the 2020 United States presidential election fraud~\cite{election_fraud} and COVID-19 rumors~\cite{covid_rumours}.
Both industry and government are making efforts to prevent the spread of fake news~\cite{fb_report}.
Nevertheless, fake news verification systems still rely on human experts and their manual efforts in analyzing the news contents with additional evidence.
To this end, there should be an automatic and efficient way to identify the veracity of the news.

The most typical way to detect fake news is applying Natural Language Processing (NLP) techniques on the news content~\cite{conroy2015automatic, feng2012syntactic}.
Considering that even people struggle in identifying the news authenticity by the news content alone, these NLP solutions are ineffective.
Thus, more information is required to improve fake news detection.
The first important information is the users in social media.
Social media is one of the most influential mediums to propagate information, and it has become a common practice for people to share their thoughts in social media.
Even though regular users use social media as a communication tool, some users, known as instigators, intentionally spread fake news.
Instigators usually have a highly partisan-biased personal description and a lot of followers and followings, which is significantly different from the profiles of regular users (See in Figure~\ref{fig:motivation}).
Therefore, analyzing the users engaged in the news can provide additional evidence for identifying news authenticity.
The publisher information can also play an important role because certain partisan-biased publishers are more likely to publish fake news~\cite{mbfc_right, mbfc_left}.
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/motivation_2.pdf}
    \caption{Publishers publish the news, and users tweet the news. Some publishers are regarded as low credibility sources according to the famous fact-checking website, MBFC. User A is an example of an instigator in Twitter, and User B is an example of a regular user.}
    \label{fig:motivation}
\end{figure}
Information on users and publishers can be viewed as multi-level social context information, and they provide additional clues for fake news detection.
A general approach to present multi-level social context is using a heterogeneous graph, where nodes are publishers, news, and users.
To fully utilize multi-level social context information in the graph and thus improve the detection performance, three chronic difficulties need to be resolved.
% we pose three crucial yet overlooked challenges.

Firstly, the multi-level social context information should be included in the news representation without information loss.
% The importance of multi-level social context information is emphasized above, and diluting such information is hard to promise a high-performing news detection.
There were several efforts to use social context information in graphs: Bi-GCN~\cite{bian2020rumor} and SAFER~\cite{chandra2020graph} use Graph Convolution Network (GCN)~\cite{kipf2016semi} to obtain the news representation with user information.
Even though they employ social user information as social context, they still suffer from information loss as they ignore the node types and relations between them.
Different node types have different kinds of information, and different relations with news indicate different aspects of news.
In this regard, the information associated with node and relation types should be preserved in the news representation.
% Tri-FN~\cite{shu2019beyond} decomposes the  to acquire the latent feature of the news with publisher and user information.
% For instance, SAFER~\cite{chandra2020graph} and Tri-FN~\cite{shu2019beyond} ignore the node types and relation types, and they apply the Graph Convolution Network (GCN)~\cite{kipf2016semi} and matrix decomposition to obtain the news representation respectively to include the social context. 

Secondly, the temporal information should be included in the news representation with multi-level social context information.
Fake and real news have different propagation properties in social media: Fake news is periodically mentioned by people and usually lasts longer, but real news receives attention only at the beginning of the news publication~\cite{kwon2013prominent}.
Due to the nature of the graph, however, temporal information is hard to present in the graph, which increases the difficulties in incorporating temporal information in the news representation with multi-level social context.
There were several works~\cite{zhou2019network, rosenfeld2020kernel} focused on the temporal information to detect fake news, but they failed to preserve all the multi-level social context information.

Lastly, the final news representation should be learned in an end-to-end manner while preserving multi-level social context information and temporal information.
Dividing into several tasks or introducing another task may cause the error propagation problem. 
FANG~\cite{nguyen2020fang}, for example, tries to preserve information by dividing the fake news detection task into several sub-tasks; if the sub-tasks, such as textual encoding and stance detection, have errors, the errors can propagate up to the final news representation and thereby affect the news detection.
% Using end-to-end learning can eliminate the effect from the sub-tasks and can optimize the training parameters with single news detection loss.
Instead of dividing the fake news detection task into several sub-tasks, we need an end-to-end method to get rid of the errors from sub-tasks and optimize the training parameters with single news detection loss.

% The distinct feature of temporal engagement of social users in real and fake news is another crucial information in fake news detection.
% It indicates that temporal feature of user engagement can also be very helpful in fake news detection task.

% In this context, we propose a novel multi-level social context aware fake news detection framework, \model{}.
% a composite relation connecting two objects, is a widely used structure to capture the semantics.
% We define two meaningful Meta-Paths to extract multi-level social context information without information loss.
% Moreover, the node features extracted from Meta-Path can be directly manipulated, which enables us to learn the news representation in an end-to-end manner.
% For temporal information of user engagement, the typical way is to feed into the Recurrent Neural Network (RNN) and capture the time series features. 
% However, in order to feed into the RNN, we first need to efficiently encode node features from Meta-Path extraction and obtain the single vector representation.
% To do this, we adopt the method from knowledge graph embedding to efficiently encode the extracted nodes following the Meta-Path.
% To tackle all these challanges, \model{} is able to produce news representation with multi-level social context information and temporal feature of user engagement in an end-to-end manner.

% It is challenging to resolve all three difficulties in a single framework.
To the best of our knowledge, existing approaches fail to address all three challenges, so we propose a novel fake news detection framework, \model{}, to tackle the above-listed challenges.
In \model{}, to preserve multi-level social context information, we use the \textit{Meta-Path} concept.
A Meta-Path is a composite relation connecting two node types, aiming at capturing the semantics in the heterogeneous graph.
%% [Definitions from other paper]
% Meta-path is a path defined on the network schema, which is a relation sequence between two object types and defines a new or existing relation between objects.
We define two Meta-Paths containing different aspects of news (users and publishers) to extract multi-level social context information without information loss.
Moreover, Meta-Path instance encoding and aggregation methods are proposed to capture the temporal information of user engagement and learn the representation end-to-end.

To show that our proposed method outperforms existing solutions, we test \model{} with two real-world datasets~\cite{nguyen2020fang, dai2020ginger}, and the results show that \model{} achieves significant improvement over previous approaches in terms of F1 score, accuracy, and AUC score. 
Our code with data is released on the GitHub~\footnote{https://github.com/(will be available)} for reproducibility. 
Our major contributions are:
\begin{enumerate}[leftmargin=.3in, topsep=3pt]
    \item We pose three crucial challenges in social context aware fake news detection and address them by proposing a novel fake news detection framework, \model{}.
    \item We conduct diverse experiments on the two real-world fake news datasets, covering the broad definition of fake news (Section~\ref{sec:preliminaries}), and demonstrate that \model{} shows better performance than existing solutions.
    \item We provide new insights into the differences in the behavior of engaged users between intentional and unintentional fake news.
\end{enumerate}

% To use both multi-level social context and temporal feature of user engagement, we design an end-to-end multi-level social context aware fake news detection framework, \model{}.
% \model{} encodes the information extracted from Meta-Path using knowledge graph embedding method, and uses Recurrent Neural Network (RNN) and attention mechanism to aggregates the representation.
% It learns the news representation containing social context in an end-to-end manner with single news detection loss.
% Recently, there were several efforts to detect fake news by presenting social context information in the graph.
% For instance, SAFER \cite{chandra2020graph} uses homogeneous graph representation and apply Graph Convolution Network (GCN)~\cite{kipf2016semi} to obtain the news representation in the graph.
% The news representation obtained from GCN is then concatenated with news content representation from pre-trained model RoBERTa~\cite{jin2020bert}.
% Tri-FN ~\cite{shu2019beyond} treats all nodes as same type and apply matrix decomposition on embedding matrix of nodes and relations to get the latent features of the news.
% FANG~\cite{nguyen2020fang} divides the fake news detection task into several sub-tasks, such as textual encoding and stance detection, and optimize them by using respective objective function.
% The user and publisher representations learned from each sub-task are then aggregate with final news detection objective to obtain the final news representation.

% All these solutions suffer from either severe information loss or error propagation problem.
% For example, SAFER and Tri-FN did not consider node types and relation types, so the information associated with node and relation types will not be included in the final news representation.
% FANG tries to preserve all the information by dividing the fake news detection task into several sub-tasks; if the sub-tasks, such as textual encoding and stance detection, have errors, the errors propagate up to the final news representation and thereby affect the news detection.
% Therefore, we need an approach that can directly extract social context information from the heterogeneous graph with minimal information loss and additional errors.
% Moreover, the connection between each type of node has different semantic meanings, so the news representation should be able to contain those meaningful semantic information as well.


% For example, Facebook encourages users to report posts that have low credibility. 
% Moreover, governments in some countries are maintaining an online fake news refutation platform to prevent people from being deceived by misinformation or disinformation~\cite{rumour_cn}. 
% Many prevalent news on the election turned out to be fake news based on insufficient evidence.
% Likewise, since the start of the COVID-19 pandemic, a surge of fake news on the coronavirus (COVID-19) appeared and caused public fear and uncertainty.
% This general spread of fake news has a direct impact on people's wellbeing~\cite{covid_who} according to the World Health Organization.
% Nevertheless, most of the fake news verification systems still rely on human experts and their manual efforts in analyzing the news contents with additional evidence. 
% To this end, there have been numerous efforts to detect fake news automatically and efficiently. 

% GNN is a class of deep learning method made for graph structural data, it has received a lot of attention due to its superior performance in some tasks for the graph, such as graph node classification and link prediction. 
% Tri-FN ~\cite{shu2019beyond} applies matrix decomposition on embedding matrix of nodes and relations to get the latent features of the news to deal with graph-structured data. 
% In order to get representations of news embedding, SAFER~\cite{chandra2020graph} concatenates the news content features from the pre-trained model RoBERTa~\cite{jin2020bert} and the graph representation from Graph Convolutional Neural Network (GCN)~\cite{kipf2016semi}. 
% The concatenated vectors are classified with Logistic Regression. 
% FANG.~\cite{nguyen2020fang} divided the fake news detection task into several sub-tasks, such as stance detection and textual encoding. 
% Thus, the representations of each type of node, user, and publisher are learned from their own sub-tasks. 
% Once the embedding of publisher and user nodes are ready, the final fake news representation is optimized by aggregating embeddings of engaged publisher and user nodes with final fake news detection loss function.

% While graph-based approaches generally gave better results than text-based approaches, existing solutions are far from mature because they still suffer from at least one of the following four major drawbacks. 
% First, most existing methods utilize matrix decomposition for graph analysis, and it is computationally expensive when handling a large number of graph nodes. 
% Second, they commonly adopt a homogeneous graph architecture when representing social media as a graph.
% This is not appropriate since graphs in the real-world are heterogeneous with diverse types of nodes and relationships.
% Third, errors from separate upstream sub-tasks, such as textual encoding and stance detection, can propagate to the final loss of fake news detection. 
% Lastly, temporal information is not considered in the final news embedding, which is important in containing the propagation property.

% These solutions were not effective, since just reading the news text (without cross-validation) cannot show whether it is true or not. 
% Some studies~\cite{forbes_study, npr_study} show that people had a hard time distinguishing fake and real news, and found that 75\% of Americans regarded fake news stories from the election as a reliable information.

% Thus, to further improve fake news detection, researchers started utilizing social media and publisher information in the form of graphs (adopting cross-validation). 
% As social media became one of the most influential mediums to propagate information, people sharing their thoughts on certain events has become common practice in social media.
% However, there exists some instigators intentionally spreading biased or fake news, so analyzing the engaged users and their reputation in the social media graph can provide additional evidence for detecting news authenticity. 
% Furthermore, the publisher information can also play an important role, because some online partisan-biased publishers are more likely to publish fake news to harm the opposing party \cite{mbfc_right, mbfc_left}. %What's more, in the recent work of Pennycook  et. al., ~\cite{pennycook2021research}, they conducted a survey about whether people believe the false claims about election fraud three days after the election, and they found out that strong minority – 40\% – still view it as truth. 
